Operator scaling: theory and applications

In this paper we present a deterministic polynomial time algorithm for testing if a symbolic matrix in non-commuting variables over $\mathbb{Q}$ is invertible or not. The analogous question for commuting variables is the celebrated polynomial identity testing (PIT) for symbolic determinants. In contrast to the commutative case, which has an efficient probabilistic algorithm, the best previous algorithm for the non-commutative setting required exponential time (whether or not randomization is allowed). The algorithm efficiently solves the "word problem" for the free skew field, and the identity testing problem for arithmetic formulae with division over non-commuting variables, two problems which had only exponential-time algorithms prior to this work. The main contribution of this paper is a complexity analysis of an existing algorithm due to Gurvits, who proved it was polynomial time for certain classes of inputs. We prove it always runs in polynomial time. The main component of our analysis is a simple (given the necessary known tools) lower bound on central notion of capacity of operators (introduced by Gurvits). We extend the algorithm to actually approximate capacity to any accuracy in polynomial time, and use this analysis to give quantitative bounds on the continuity of capacity (the latter is used in a subsequent paper on Brascamp-Lieb inequalities). Symbolic matrices in non-commuting variables, and the related structural and algorithmic questions, have a remarkable number of diverse origins and motivations. They arise independently in (commutative) invariant theory and representation theory, linear algebra, optimization, linear system theory, quantum information theory, approximation of the permanent and naturally in non-commutative algebra. We provide a detailed account of some of these sources and their interconnections.

==> probdefs.tex <==

In this section we define more formally the various reincarnations, in different mathematical areas, of the problem SINGULAR solved by algorithm $G$. We start in Subsection~\ref{prelim:defs} with more formal definitions of the necessary concepts from these various areas (many given semi-formally in the introduction), proceed in Subsection~\ref{prob:defs} with formal definitions of the problem in each area, and conclude with a formal statement of what Algorithm $G$ achieves for all.

\subsection{Preliminary definitions}\label{prelim:defs}



\subsubsection{Free Skew Field}\label{freeskewprelims}

Let $\bx = \{x_1, \ldots, x_m \}$ be a set of non-commuting variables. We will denote by $\mathbb{F} \langle \bx \rangle$, the ring of polynomials 
in non-commuting variables $x_1,\ldots,x_m$ over the (commuting) field $\mathbb{F}$. We will denote by 
$\mathbb{F} \langC \bx \rangC$, the free skew (non-commutative) field of rational functions in non-commuting variables 
$x_1,\ldots,x_m$ over the (commuting) field $\mathbb{F}$. We will describe below the original construction of 
Amitsur \cite{amitsur66} to describe this skew field. 

A non-commutative circuit $\Phi$ (with inversions) over a (commutative) field $\mathbb{F}$ and non-commuting variables $x_1,\ldots,x_m$ is a directed acyclic graph. Nodes of in-degree zero are labelled by a variable or a field element from $\mathbb{F}$. Nodes of in-degree one are labelled by $^{-1}$ and nodes of in-degree two are labelled by a $+$ or $\times$. The two edges going into a node labelled by $\times$ are labelled {\em left} and {\em right} to specify the order of multiplication. The nodes are called input gates, inverse gates and sum and product gates respectively. The nodes of out-degree zero are called output gates. The size of a circuit $\Phi$ is the number of gates in it. A formula is a circuit all of whose nodes/gates have out-degree at most one. 

A node $v \in \Phi$ is supposed to compute a non-commutative rational function 
$\hat{v} \in \mathbb{F} \langC \bx\rangC$. However $\Phi$ may contain division by zero, in which case $\hat{v}$ would be undefined. 
The definition of $\hat{v}$ is the following:
\begin{enumerate}
\item If $v$ is an input gate, labelled by $a$ (variable or a field element), then $\hat{v} \coloneqq a$.
\item If $v$ is a sum or a product gate and $v = v_1 + v_2$ or $v = v_1 \times v_2$, then $\hat{v} \coloneqq \hat{v_1}+\hat{v_2}$ or $\hat{v} \coloneqq \hat{v_1} \times \hat{v_2}$ respectively and assuming that $\hat{v_1}$ and $\hat{v_2}$ are both defined.
\item If $v$ is an inverse gate and $v = u^{-1}$, then $\hat{v} \coloneqq \hat{u}^{-1}$ if $\hat{u}$ is defined and $\hat{u} \neq 0$. 
\end{enumerate}

\noindent We say that $\Phi$ is a {\em correct circuit} if $\hat{u}$ is defined for every gate $u \in \Phi$. 
%Some examples of non-commuting rational expressions are $(xy - yx)^{-1}, (xu^{-1}z + y)^{-1}, (x+y)^{-1} - x^{-1}$. 

\noindent Note that unlike the commutative case, a non-commutative rational expression might not be expressible as a ratio of two polynomials 
and in fact, there could be an unbounded number of nested inversions in such expressions~\cite{Reut96}. But still there are nontrivial 
rational identities in the non-commutative setting. One example is Hua's identity \cite{Hua}, $(x+ xy^{-1}x)^{-1}$ is equivalent to the expression 
$x^{-1} - (x+y)^{-1}$. So it is highly nontrivial to even define the free skew field. The first construction of the free skew field was given by 
Amitsur~\cite{amitsur66}. Subsequently, alternate constructions were given by Bergman~\cite{bergman}, Cohn~\cite{cohn1971-sf}, 
Malcolmson~\cite{malcolmson}. 

Let $\Phi$ be a circuit and $(B_1,\ldots,B_m)$ be a tuple of matrices. Then we will say that $\Phi$ is defined on $(B_1,\ldots,B_m)$ if all the inversions in $\Phi$ are possible when evaluated on $B_1,\ldots,B_m$. Amitsur proved that the set of all circuits (or equivalently formulas) modulo this equivalence relation form a skew field.

\begin{definition} Let $\Phi$ be a non-commutative circuit with inversions. 
$$
\text{Dom}(\Phi) \coloneqq \{ (B_1,\ldots,B_m) : \text{$\Phi$ defined on $(B_1,\ldots,B_m)$}\}
$$
\end{definition}

\noindent Two circuits $\Phi_1$ and $\Phi_2$ are said to be equivalent if $\hat{\Phi}_1(B_1,\ldots,B_m) = \hat{\Phi}_2(B_1,\ldots,B_m)$ for all $(B_1,\ldots,B_m) \in$ $\text{Dom}(\Phi_1) \cap \text{Dom}(\Phi_2)$ (and $\text{Dom}(\Phi_1) \cap \text{Dom}(\Phi_2) \neq \phi$). 


\noindent We refer the reader to \cite{vinnikov10, HW14} and references therein for further information 
about the free skew field.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Shrunk Subspace}

The notion of a shrunk subspace will be very crucial for us.

\begin{definition} Let $A_1,\ldots, A_m \in M_n(\F)$. $A_1,\ldots, A_m$ are said to admit a shrunk subspace if there exist subspaces $V, W \subseteq \mathbb{F}^n$ s.t. $\dim(W) < \dim(V)$ and $A_i(V) \subseteq W$ for $1 \le i \le m$ ($V$ is the shrunk subspace here, shrunk to $W$ simultaneously by all $A_i$). $A_1,\ldots, A_m$ are said to admit a $c$-shrunk subspace if there exist subspaces $V, W \subseteq \mathbb{F}^n$ s.t. $\dim(W) \le \dim(V) - c$ and $A_i(V) \subseteq W$ for $1 \le i \le m$. 
\end{definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Invariant Theory}{\label{InvTheory}}

In this section, we give the relevant background from Invariant Theory. We will give only a high level overview needed to understand the problems and the results in this paper. One can find much more in the books \cite{Kraft-Procesi, Derksen-Kemper}. In this section, all the variables {\em commute}!

\noindent Fix a field $\mathbb{F}$. Let $G$ be a group and $V$ be its representation, namely a vector space on which $G$ acts. The group 
$G$ then also acts on the polynomial functions on $V$, $\mathbb{F}[V]$, which is also called the {\em coordinate ring} of $V$. In our case 
$V$ will be finite dimensional (say $m$), so $\mathbb{F}[V]$ will be simply be $\mathbb{F}[\by]$, where $\by = \{y_1,\ldots,y_m\}$.  
For a polynomial $p(\by) \in \mathbb{F}[\by]$, we will denote by $g p$ the action of $g \in G$ on $p$. A polynomial is said to be 
invariant if $g p = p$ for all $g \in G$. The following is a well studied example:

\begin{example} Let $G = S_m$ acts on the set of formal variables $\by$ (and hence on the vector spaces defined by them) by 
permuting them. Then the set of invariant polynomials are all the symmetric polynomials.
\end{example}

The \emph{null-cone} of an action is the set of all common zeroes of the non-constant invariant polynomials of the action.

We will be interested in the so called left-right action. Here a pair of matrices $(B,C) \in SL_n(\F) \times SL_n(\F)$ acts on 
$(X_1,\ldots, X_m)$ to give $(BX_1C,\ldots, BX_mC)$. The variables are the entries of $X_1,\ldots,X_m$, so there are 
$m n^2$ variables in total. 

\noindent Explicit generating sets for the invariant ring of polynomials of the left-right action have been well studied and the following 
is known about them:

\begin{theorem}[\cite{DW2000, DZ2001, SVdB2001, ANS10}] Over algebraically closed fields $\mathbb{F}$, the set 
$$
\left\{ \Det\left( \sum_{i=1}^m X_i \tensor B_i \right): k \in \mathbb{N}, B_i \in M_k(\mathbb{F}) \right\}
$$
is a generating set for the ring of invariant polynomials of the left-right action.
\end{theorem}

\noindent These are in fact special cases of more general results on invariant rings of arbitrary quivers. Explicit exponential bounds on the degree of polynomials required to generate the ring of invariant polynomials are known. It is in fact a very important open problem to obtain polynomial degree bounds for the generating set. See \cite{HW14} for some applications which include eliminating divisions from non-commutative circuits.

\noindent The null-cone of the left-right action (over algebraically closed fields of arbitrary characteristic) was studied 
in~\cite{BD06, ANS10}, who proved the following theorem:

\begin{theorem}[\cite{BD06, ANS10}]{\label{null-cone-shrunk}} $(A_1,\ldots,A_m)$ is in the null-cone of the left-right action iff 
$A_1,\ldots,A_m$ admit a shrunk subspace.
\end{theorem}

\noindent We state the degree bounds for the generating set of invariant polynomials in terms of the dimension of matrices required to 
test the null-cone property. But these are essentially equivalent to the degree bounds by~\cite{derksen} (over algebraically closed fields of characteristic zero). 

\begin{theorem}[\cite{derksen}] Let $A_1,\ldots, A_m$ be $n \times n$ complex matrices such that they 
are not in the null-cone of the left-right action. Then there exist matrices $B_1,\ldots, B_m$ of dimension 
$n^2 4^{n^2}$ s.t. 
$$
\Det \left( A_1 \tensor B_1 + \cdots A_m \tensor B_m \right) \neq 0
$$ 
\end{theorem}

\begin{theorem}[\cite{IQS2015}]{\label{IQS}} Let $A_1,\ldots, A_m$ be $n \times n$ complex 
matrices that are not in the null-cone of the left-right action. Then there exist matrices $B_1,\ldots, B_m$
of dimension $(n+1)!$ s.t. 
$$
\Det \left( A_1 \tensor B_1 + \cdots A_m \tensor B_m \right) \neq 0
$$ 
\end{theorem}

\noindent There has been remarkable progress on this problem recently. 

\begin{theorem}[\cite{derksen2015, IQS15b}]{\label{new_bounds}} Let $A_1,\ldots, A_m$ be $n \times n$ complex 
matrices that are not in the null-cone of the left-right action. Then there exist matrices $B_1,\ldots, B_m$
of dimension $n-1$ s.t. 
$$
\Det \left( A_1 \tensor B_1 + \cdots A_m \tensor B_m \right) \neq 0
$$ 
\end{theorem}

\noindent By combining Theorem \ref{null-cone-shrunk} and Theorem \ref{new_bounds}, we get the following theorem:

\begin{theorem}{\label{fullness_dimension}} Let $A_1,\ldots, A_m$ be $n \times n$ complex 
matrices such that they do not admit a shrunk subspace. Then there exist matrices $B_1,\ldots, B_m$
of dimension $n-1$ s.t. 
$$
\Det \left( A_1 \tensor B_1 + \cdots A_m \tensor B_m \right) \neq 0
$$ 
\end{theorem}

\subsection{Problem Definitions}\label{prob:defs}




In this section, we formally state and give some background to 
all incarnations of the problems solved by Algorithm G. These problems arise from several 
disparate fields which are all magically interconnected. In most of these problems, the inputs 
will essentially be a tuple of $n \times n$ matrices with rational entries $A_1,\ldots,A_m$. We will denote 
the maximum bit size of the entries of these matrices by $b$. We give 
deterministic $\text{poly}(n,m,b)$ time algorithms for all of these problems.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{SINGULAR}

In the (non-commutative) SINGULAR problem, the input is a matrix $L \in M_n(\F\la \bx \ra)$ whose entries are linear polynomials and the 
question is to check whether $L$ is singular (not invertible) over $\F \langC \bx \rangC$. The problem makes sense over any field but 
our results will hold when $\mathbb{F} = \mathbb{Q}$ (most of the theory works over $\mathbb{C}$ but to account for input size, 
we only work over the rationals).

\begin{problem}\label{prob:singular} SINGULAR \\
\textbf{Input}: $A_1,\ldots,A_m \in M_n(\mathbb{Q})$ interpreted as $L = \sum_{i=1}^m x_i A_i$ \\
\textbf{Output}: Is $L$ singular over the free skew field $\Qxx$? \\
%\textbf{Input size}: $n + b$
\end{problem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Computing the Non-Commutative Rank and Fullness Testing}\label{def:ncrank}

We also study the problem of computing the rank of a matrix over the free skew field. It turns out that there are various 
interesting notions of rank which coincide. The two main ones for us will be the inner rank and the rank over the free skew field 
(which is unambiguously defined). 

\begin{definition}[Inner Rank] Suppose $L$ is a matrix in $\mathbb{F} \la \bx \ra^{n \times p}$. The inner rank of $L$ is 
defined as the minimum $r$ such that $L = K M$, where $K \in \mathbb{F} \la \bx \ra^{n \times r}$ and 
$M \in \mathbb{F} \la \bx \ra^{r \times p}$.
\end{definition}

It is clear that the inner rank of $L$ is at most $\min(n,p)$, since we can write $L = I_n \cdot L$ and $L = L \cdot I_p$. 
When the inner rank of $L$ is equal to $\min(n, p)$, we say that $L$ is a {\em full matrix}. 
The more formal definition is given below:

\begin{definition}[Fullness] A matrix $L \in M_n(\F \la \bx \ra)$ is said to be {\em full} if it cannot be written as 
$$
L = K M
$$
where $K\in \F \la \bx \ra^{n \times r}$, $M \in \F \la \bx \ra^{r \times n}$, for some $r < n$. 
\end{definition} 

The other way to define the non-commutative rank of a matrix $L$ is by defining its rank over the free skew field, which
we do now.

\begin{definition}\label{def:NCrank}[Non-Commutative Rank] Given a matrix $L$ in $\mathbb{F} \la \bx \ra^{n \times p}$, $\ncrk(L)$ is 
defined to be the rank of $L$ over $\mathbb{F} \langC \bx \rangC$.
\end{definition}

It is important to notice that even over skew fields, the rank of a matrix is defined 
unambiguously as the row rank or the column rank.

Now that we have defined the non-commutative rank of a matrix, we state the general problem of determining the
non-commutative rank of matrices over $\FX$.

\begin{problem}\label{prob:NCrank} Computing Noncommutative rank \\
\textbf{Input}: Matrix $L$ in $\mathbb{Q} \la \bx \ra^{n \times p}$.  Each entry is given by a formula computing it which is of 
size $s$ and uses field elements (rational numbers) of bit size at most $b$. \\
\textbf{Output}: $\ncrk(L)$ \\
\textbf{Input size}: $n + p+ b + s$. 
\end{problem}

Since we can compute the non-commutative rank of $L$, we can also determine whether $L$ is full. Thus, by solving
Problem~\ref{prob:NCrank} we have solved the following problem:

\begin{problem}\label{prob:gen-fullness} General Fullness testing \\
\textbf{Input}: Formulas computing the entries of a matrix $M \in M_n(\FX)$. \\
\textbf{Output}: Is $M$ full? \\
\end{problem}


Due to the following theorem of Cohn, which works over all fields, by testing fullness of a matrix
we can also decide whether a matrix is invertible over the free skew field:

\begin{theorem}[\cite{Cohn-SF}]{\label{inv_to_full}}
Let $L \in \mathbb{F} \la \bx \ra^{n \times n}$. Then $L$ is invertible over 
$\F \langC \bx \rangC$ if and only if $L$ is full.
\end{theorem}

It is important to remark that the analogous statement for matrices of commutative polynomials is not true. 
The following skew symmetric matrix is a counterexample:
\[
  \begin{bmatrix}
    0 & x & y \\
    -x & 0 & 1 \\
    -y & -1 & 0
  \end{bmatrix}
\] 
\noindent It is full but not invertible (when $x$ and $y$ are commuting variables).

Going back to Definition~\ref{def:NCrank}, let us assume for the sake of simplicity that $L$  is square, i.e. $n=p$, 
although the results hold for rectangular matrices as well.

As stated in Theorem \ref{cohn-nc=inner}, Cohn proved that $\ncrk(L)$ is equal to the inner rank of $L$ (there it is stated for 
$L$ which have linear polynomials as entries but it is in fact true for general $L$ as seen by the Higman's trick (see section \ref{computeNC}) 
of reducing general $L$ to the linear case). Theorem \ref{cohn-nc=inner} also states that a linear matrix $L$ has $\ncrk(L) \le r$ iff there 
exist invertible matrices $B,C$ over $\mathbb{F}$ s.t. $BLC$ has a block of zeroes of size $i \times j$ where $i + j \ge 2n-r$. This can 
be easily translated into the following theorem:

\begin{theorem} A linear matrix $L = \sum_{i=1}^m x_i A_i \in M_n(\mathbb{F} \la x_1,\ldots,x_m\ra)$ has $\ncrk(L) \le r$ iff $A_1,\ldots,A_m$ 
admit a $n-r$-shrunk subspace. 
\end{theorem}

\noindent By proposition \ref{shrunk=decreasing}, we also get that a linear matrix $L = \sum_{i=1}^m x_i A_i \in M_n(\mathbb{F} \la \bx \ra)$ 
has $\ncrk(L) \le r$ iff the operator defined by $A_1,\ldots,A_m$ is $(n-r)$-rank-decreasing. In section \ref{computeNC}, we will give two 
different deterministic polynomial time algorithms for computing noncommutative rank, one by an algebraic reduction to fullness testing 
and the other via a ``quantum" reduction from checking if an operator is $c$-rank-decreasing to checking if an operator is rank-decreasing.



%\begin{definition} A matrix $L \in M_n(\F \la \bx \ra)$ is said to be full if it cannot be written as 
%$$
%L = K M
%$$
%where $K\in \F \la \bx \ra^{n \times r}$, $M \in \F \la \bx \ra^{r \times n}$, for some $r < n$. 
%\end{definition} 
%
%\begin{problem}\label{prob:fullness} Fullness testing \\
%\textbf{Input}: $A_1,\ldots,A_m \in M_n(\Q)$ interpreted as $L = \sum_{i=1}^m x_i A_i$. \\
%\textbf{Output}: Is $L$ full? \\
%\end{problem}
%
%More generally, due to Higman's trick~\ref{prop:higman-trick}, we can reduce the more general
%problem of testing whether a matrix with polynomial entries, whose entries are 
%computed by small formulas, is full, to the problem of testing fullness of a matrix with linear entries.
%Thererefore, Algorithm G will also solve the following more general problem:
%
%
%\begin{problem}\label{prob:gen-fullness} General Fullness testing \\
%\textbf{Input}: Formulas computing the entries of a matrix $M \in M_n(\FX)$. \\
%\textbf{Output}: Is $M$ full? \\
%\end{problem}
%
%
%\noindent Cohn proved the following theorem (works over all fields):
%
%\begin{theorem}[\cite{Cohn-SF}]{\label{inv_to_full}}
%Let $L \in \mathbb{F} \la x_1,\ldots,x_m\ra^{n \times n}$. Then $L$ is invertible over 
%$\F \langC \bx \rangC$ if and only if $L$ is full.
%\end{theorem}
%
%\noindent The analogous statement for matrices of commutative polynomials is not true. 
%The following skew symmetric matrix is a counterexample:
%\[
%  \begin{bmatrix}
%    0 & x & y \\
%    -x & 0 & 1 \\
%    -y & -1 & 0
%  \end{bmatrix}
%\] 
%\noindent It is full but not invertible (when $x$ and $y$ are commuting variables).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Testing Shrunk Subspaces}


\begin{problem}\label{prob:shrunk} Testing shrunk subspaces \\
\textbf{Input}: $A_1,\ldots,A_m \in M_n(\Q)$. \\
\textbf{Output}: Do $A_1,\ldots, A_m$ admit a shrunk subspace? \\
\end{problem}

\noindent Another theorem due to Cohn is the following (works over all fields):

\begin{theorem}[\cite{Cohn-SF}]{\label{full_to_Hall}}
A matrix $L = \sum_{i=1}^m x_i A_i \in M_n(\F \la \bx \ra)$ is not full if and only if there are invertible matrices 
$U, V \in M_n(\mathbb{F})$ s.t. $U L V$ has a $r \times s$ block of zeroes for some $r,s$ with $r + s > n$.
\end{theorem}

\noindent The above theorem is an analogue of Hall's bipartite matching theorem where the $r \times s$ block of zeroes corresponds to a set of size $r$ on one side of the bipartition and set of size $s$ on the other side of the bipartition with no edges between them. If $r + s > n$, this prevents the graph from having a perfect matching. The following theorem is an easy corollary of Theorem \ref{full_to_Hall}. 
%The analogue of a shrunk subset i.e. a set of vertices $S$ on one side of the bipartition s.t. $|N(S)| < |S|$ ($N(S)$ is the set of neighbors of $S$) is taken by shrunk subspaces and 

\begin{theorem}{\label{full_to_shrunk}}
A matrix $L = \sum_{i=1}^m x_i A_i \in M_n(\mathbb{F} \la \bx \ra)$ is not full if and only if $A_1,\ldots, A_m$ admit a shrunk subspace.
\end{theorem}

\noindent So an extremely hard looking problem about inverting matrices in the free skew field is equivalent to a simply stated problem in (commutative) linear algebra! 

\begin{remark}{\label{QvsC}}
$A_1,\ldots, A_m$ shrink a subpace of $\mathbb{C}^n$ iff $A_1,\ldots,A_m$ shrink a subspace of $\mathbb{Q}^n$ since 
$\sum_{i=1}^m x_i A_i$ is invertible over $\mathbb{C} \langC \bx \rangC$ iff it is invertible over 
$\mathbb{Q} \langC \bx \rangC$.
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Null-Cone of the Left-Right Action}

\begin{problem}\label{prob:null} Testing membership in the null-cone of the left-right action \\
\textbf{Input}: $A_1,\ldots, A_m \in M_n(\Q)$. \\
\textbf{Output}: Does $(A_1,\ldots, A_m)$ lie in the null-cone of the left-right action? \\
%\textbf{Input size}: $n + b$, where $b$ is the maximum number of bits needed to represent any entry in $A_1,\ldots, A_m$.
\end{problem}

\noindent As we saw in section \ref{InvTheory}, testing if $(A_1,\ldots,A_m)$ is in the null-cone of the left-right action is the same as testing if $A_1,\ldots,A_m$ admit a shrunk subspace (over algebraically closed fields). 

\begin{theorem}[\cite{BD06, ANS10}]{\label{null-cone-shrunk}} $(A_1,\ldots,A_m)$ is in the null-cone of the left-right action iff 
$A_1,\ldots,A_m$ admit a shrunk subspace.
\end{theorem}

\noindent The above theorem can also be obtained in a round-about manner through infinite generating sets of the left-right action. 
The tuple $(A_1,\ldots,A_m)$ is in the null-cone of the left-right action iff 
$$
\Det\left( \sum_{i=1}^m A_i \tensor B_i \right) = 0
$$
for all $k \in \mathbb{N}, B_i \in M_k(\mathbb{F})$. This is equivalent to the matrix $\sum_{i=1}^m x_i A_i$ being singular over the free 
skew field $\mathbb{F} \langC \bx \rangC$ (this essentially follows from Amitsur's construction of the free skew field~\cite{amitsur66}, 
see~\cite{HW14}) which is equivalent to $A_1,\ldots,A_m$ admitting a shrunk subspace, because of Theorem~\ref{inv_to_full} and 
Theorem~\ref{full_to_shrunk}. 

\noindent In \cite{ANS10}, several fundamental problems about the left-right action were connected to Geometric Complexity Theory. 
Most of these problems seem to require polynomial degree bounds for the generating set of the invariant ring of polynomials. However, 
we are able to bypass proving these polynomial degree bounds for determining membership in the null-cone over $\mathbb{Q}$, 
and it is plausible that our methods can solve other problems for the left-right action, e.g. the orbit closure intersection problem.

\subsubsection{Testing Rank Decreasing Property of Quantum Operators}
This problem will only make sense over $\mathbb{Q}$ (or more generally over $\mathbb{C}$). 

\begin{definition} A completely positive operator is called rank decreasing if there exists a $X \succeq 0$ s.t. 
$$
\text{Rank}(T(X)) < \text{Rank(X)}
$$
\end{definition}

\noindent We will restrict our attention quantum operators with Kraus operators having rational entries.

\begin{problem}\label{prob:quantum} Testing if quantum operators are rank decreasing \\
\textbf{Input}: $A_1,\ldots,A_m$ interpreted as a quantum operator $T$ with Kraus operators $A_1,\ldots,A_m$.\\
\textbf{Output}: Is $T$ rank decreasing? \\
%\textbf{Input size}: $n+b$, where $b$ is the maximum bit size of entries in $A_1,\ldots,A_m$.
\end{problem}

\begin{proposition} [\cite{gurvits2004}]\label{shrunk=decreasing}
Suppose $T$ is a cptp map whose Kraus operators are $A_1,\ldots, A_m$. Then $T$ is $c$-rank-decreasing iff $A_1,\ldots, A_m$ admit a $c$-shrunk subspace.
\end{proposition}

\noindent The connection essentially is that if $A_1,\ldots,A_m$ shrink a subspace $V$, then $T$ will decrease the rank of the projector onto $V$, $\Pi_V$. 

\begin{proof}
First suppose that $A_1,\dots, A_m$ have a shrunk subspace $V$ such that each $A_i$ maps $V$ into $W$, where $\text{dim}(W) \le \text{dim}(V)-c$. Suppose $\text{dim}(V) = p$ and $v_1,\ldots,v_p$ be an orthonormal basis for $V$. Let $\Pi_V$ be the projection onto $V$. Then $\text{Rank}(\Pi_V) = p$. We will show that $\text{Rank}(T(\Pi_V)) \le p-c$ which will show that $T$ is $c$-rank-decreasing. 
\begin{align*}
T(\Pi_V) = \sum_{i=1}^m \sum_{j=1}^p A_i v_j v_j^{\dagger} A_i^{\dagger}
\end{align*}
Since for all $i, j$, $A_i v_j \in W$, it is clear that $\text{Im}(T(\Pi_V)) \subseteq W$ and hence $\text{Rank}(T(\Pi_V)) \le p-c$. 

Now suppose that $T$ is $c$-rank-decreasing i.e. there exists a hermitian $X$, $X \succeq 0$ s.t. $\text{Rank}(T(X)) \le \text{Rank}(X)-c$. We will show that $\text{Im}(X)$ is a $c$-shrunk subspace for $A_1,\ldots, A_m$. For this it suffices to show that for all $i$, $A_i (\text{Im}(X)) \subseteq \text{Im}(T(X))$. This is true because:

\begin{align*}
A_i (\text{Im}(X)) = A_i (\text{Im}(X^{1/2})) &= \text{Im}(A_i X^{1/2}) \\
&= \text{Im}(A_i X A_i^{\dagger}) \\
&\subseteq \text{Im}\left( \sum_{j=1}^m A_j X A_j^{\dagger} \right) \\
&= \text{Im}(T(X))
\end{align*}
The third equality follows from the fact that $\text{Im(A)} = \text{Im}(A A^{\dagger})$ for any matrix $A$. The containment follows from the following claim:

\begin{claim} Let $A$ and $B$ be two psd matrices. Then $\text{Im}(A) \subseteq \text{Im}(A + B)$.
\end{claim}

\begin{proof}
Suppose $\text{Im}(A) \subseteq \text{Im}(A + B)$ is not true. Then there exists a vector $u$ s.t. $u^{\dagger} A u > 0$ but  $u^{\dagger} (A+B) u = 0$, which is clearly not possible since $u^{\dagger} B u \ge 0$. 
\end{proof}
\end{proof}

\begin{remark} Because of Remark \ref{QvsC}, $T$ decreases the rank of a psd matrix with rational entries iff it decreases the rank of a psd matrix with complex entries.
\end{remark}

\subsubsection{Matrix Inverse Identity Testing}

INVERSE is the following computational model: Given a matrix $L \in M_n(\Fx)$ whose entries are linear polynomials ($L = A_1 + \sum_{i=2}^m x_i A_i$), the output is the top right entry of $L^{-1}$ ($A$ should be invertible over the free skew field $\Fxx$). Note that the output is a rational function in the non-commuting variables $\bx = x_1,\ldots, x_m$. This model is exponentially more powerful than non-commutative formulas with divisions \cite{HW14}, can (efficiently) simulate non-commutative algebraic branching programs (without division) \cite{HW14} and can be (efficiently) simulated by non-commutative circuits with division \cite{HW14}. However it is not known whether INVERSE can simulate non-commutative circuits (with or without division) or not. 

\noindent We are interested in the identity testing of INVERSE, namely given an invertible (over $\Fxx$) linear matrix $L$ as input, check whether the top right entry of $L^{-1}$ is zero. It is worth noting that the word problem for this computational model, whether, given two linear matrices $L$ and $M$, the top right entries of $L^{-1}$ and $M^{-1}$ are the same or not, can be reduced to the identity testing problem. The difference between the top right entries of $L^{-1}$ and $M^{-1}$ can be written as the top right entry of $N^{-1}$ for a slightly larger linear matrix $N$ \cite{HW14}.

The problem makes sense for any underlying field $\mathbb{F}$. However our results will hold for $\mathbb{F} = \mathbb{Q}$.

\begin{problem}{\label{prob_matinv}} INVERSE identity testing \\
\textbf{Input}: $A_1,\ldots,A_m$ interpreted as $L = A_1 + \sum_{i=2}^m x_i A_i$. \\
\textbf{Ouput}: Is the top right entry of $L^{-1}$ zero? \\
%\textbf{Input size}: $n + b$, where $b$ is the maximum number of bits needed to represent any entry in $A_0,A_1,\ldots, A_m$.
\end{problem}

\noindent In \cite{HW14}, it was shown that INVERSE identity testing can be reduced to SINGULAR. Let $u$ be the $1 \times n$ vector $(1,0,\ldots,0)$ and $v$ be $(0,0,\ldots,1)$. 

\begin{proposition}[\cite{HW14}] Suppose $L \in M_n(\Fx)$ is invertible (over $\Fxx$). Then the top right entry of $L^{-1}$ is zero iff 
\[
M = \begin{bmatrix}
     v^T \:\:\:L \\
     0    \:\:\:-u
    \end{bmatrix}
\]
is singular.
\end{proposition}

\noindent Previously we only considered singularity testing for matrices of the form $\sum_{i=1}^m x_i B_i$ but now we are looking at matrices of the form $B_1 + \sum_{i=2}^m x_i B_i$. However $B_1 + \sum_{i=2}^m x_i B_i$ is singular iff $\sum_{i=1}^m x_i B_i$ is singular. This is best seen from the shrunk subspace perspective, these matrices are singular iff $B_1,\ldots,B_m$ admit a shrunk subspace.


\subsubsection{Non-commutative Rational Identity Testing}
In this section, we look at the problem of non-commutative rational identity testing (RIT) of formulas. Given an element of the free skew field $\Fxx$, represented as a formula over non-commutative variables with addition, multiplication and inversion gates, we want to check if the element is zero or not. Note that the word problem over the free skew field, where we are given two rational expressions (represented as formulas) and want to check if they represent the same element in the free skew field, can be easily reduced to non-commutative RIT. 

\begin{problem}\label{prob:RIT} Non-commutative RIT \\
\textbf{Input}: Non-commutative formula $\Phi$ (with inversion gates) of size $s$. \\
\textbf{Output}: Does $\Phi$ represents zero or not? \\
\textbf{Input size}: $s+b$, where $b$ is the maximum bit size of field elements (rational numbers) used in the formula.
\end{problem}

\noindent Non-commutative RIT can be reduced to INVERSE identity testing because of the following theorem.

\begin{theorem}[\cite{HW14}] For each non-commutative formula (with inversions) $\Phi$ whose size is $s$ and uses rational numbers of bit size at most $b$, there exists $s' \le 2s$ and a $s' \times s'$ matrix $L_{\Phi}$, whose entries are either variables or rational numbers of bit size at most $b$ such that the rational functions computed by $\Phi$ and the top right entry of $L_{\Phi}^{-1}$ are the same. 
\end{theorem}

\subsection{Results}

\begin{theorem}{\label{thm:algs}} There are deterministic polynomial time algorithms for Problems \ref{prob:singular}, %\ref{prob:fullness}, 
\ref{prob:shrunk}, \ref{prob:null}, \ref{prob:quantum}, \ref{prob:NCrank}, \ref{prob_matinv},
\ref{prob:RIT}. For problems \ref{prob:singular}, %\ref{prob:fullness}, 
\ref{prob:gen-fullness}, \ref{prob:shrunk}, \ref{prob:null}, 
\ref{prob:quantum}, \ref{prob_matinv}, the complexity is $\poly(n,b)$. For \ref{prob:NCrank}, the complexity is $\poly(n,p,s,b)$, 
whereas for \ref{prob:RIT}, it is $\poly(s,b)$. 
\end{theorem}
